On the Optimality of the Kautz-Singleton Construction in Probabilistic Group Testing

We consider the probabilistic group testing problem where $d$ random defective items in a large population of $N$ items are identified with high probability by applying binary tests. It is known that $\Theta(d \log N)$ tests are necessary and sufficient to recover the defective set with vanishing probability of error when $d = O(N^{\alpha})$ for some $\alpha \in (0, 1)$. However, to the best of our knowledge, there is no explicit (deterministic) construction achieving $\Theta(d \log N)$ tests in general. In this work, we show that a famous construction introduced by Kautz and Singleton for the combinatorial group testing problem (which is known to be suboptimal for combinatorial group testing for moderate values of $d$) achieves the order optimal $\Theta(d \log N)$ tests in the probabilistic group testing problem when $d = \Omega(\log^2 N)$. This provides a strongly explicit construction achieving the order optimal result in the probabilistic group testing setting for a wide range of values of $d$. To prove the order-optimality of Kautz and Singleton's construction in the probabilistic setting, we provide a novel analysis of the probability of a non-defective item being covered by a random defective set directly, rather than arguing from combinatorial properties of the underlying code, which has been the main approach in the literature. Furthermore, we use a recursive technique to convert this construction into one that can also be efficiently decoded with only a log-log factor increase in the number of tests.

==> algorithm.tex <==
\include{algorithmic}
\include{algorithm}

\begin{algorithm}[ht]
	\caption{Alternating minimax privacy preserving algorithm}\label{alg:euclid}
	\begin{algorithmic}
		\STATE \textit{Input:} dataset $\mathcal{D}$, distortion parameter $D$, iteration number $T$\\
		\STATE \textit{Output:} Optimal privatizer parameter $\theta_{p}$\\
		%\STATE \textbf{procedure: }{Alernate Minimax}{$\mathcal{D}, D, T$}\\
		\STATE Initialize $\theta^1_{p}$ and $\theta^1_{a}$\\
		\FOR {$t=1,...,T$}
		\STATE Random minibatch of $M$ datapoints $\{x_{(1)},...,x_{(M)}\}$ drawn from full dataset\\
		\STATE Generate $\{\hat{x}_{(1)},...,\hat{x}_{(M)}\}$ via $\hat{x}_{(i)}=g(x_{(i)};\theta^t_{p})$ \\
		\STATE Update the adversary parameter $\theta^{t+1}_a$ by stochastic gradient ascend for $k$ epochs
		{$$\quad \theta^{t+1}_a=\theta^{t}_a+\alpha_t\nabla_{\theta_a} \frac{1}{M}\sum\limits_{i=1}^{M}-\ell(h(\hat{x}_{(i)};\theta_{a}),y_{(i)}), \quad\alpha_t>0$$}
		\STATE Compute the descent direction $\nabla_{\theta_{p}} l(\theta_{p}, \theta^{t+1}_a)$, where
		{$$
			\nonumber
			\ell(\theta_{p},\theta^{t+1}_a)= -\frac{1}{M}\sum\limits_{i=1}^{M}\ell(h(g(x_{(i)};\theta_{p});\theta^{t+1}_a),y_{(i)})
			$$}
		\quad\qquad subject to $ \frac{1}{M}\sum_{i=1}^{M}[d(g(x_{(i)}; \theta_{p}), x_{(i)})]\le D$\\
		\STATE Perform line search along $ \nabla_{\theta_{p}} l(\theta_{p}, \theta^{t+1}_a)$ and update
		$$\theta^{t+1}_{p}= \theta^{t}_{p}-\alpha_t \nabla_{\theta_{p}} \ell(\theta_{p}, \theta^{t+1}_a)$$
		\STATE Exit if solution converged\\
		\ENDFOR
		\STATE \textbf{return} $\theta^{t+1}_p$\\
	\end{algorithmic}
\end{algorithm}

